RoboSense: Leveraging Robotaxi Fleets as Drive-by Sensors for Urban Traffic Monitoring

Urban traffic monitoring plays a critical role in safety analysis, congestion management, and incident response. The growing deployment of robotaxis creates a new opportunity for network-level traffic monitoring. Although robotaxis are primarily designed to serve passengers, they can also be leveraged as drive-by sensors to collect traffic data. Compared to conventional infrastructure sensors or probe vehicles, a fleet of robotaxis forms a cooperative perception environment, which can collectively gather spatially and temporally continuous traffic information. This paper proposes a novel dynamic robotaxi routing framework that explicitly incorporates traffic monitoring tasks as an objective. The framework introduces: (1) a cell-based network representation that aligns with sensing capabilities of robotaxis; (2) a cell-level monitoring metric to quantify spatiotemporal robotaxi coverage; and (3) a mixed-integer linear programming (MILP) formulation that jointly minimizes time-dependent travel time and maximizes traffic monitoring performance. A 5 by 5 urban grid network is built in SUMO to evaluate the framework under three robotaxi market penetration rates (2%, 5%, and 10%) with a range of objective weight combinations. Results show that incorporating spatiotemporal network coverage in the objective function can effectively improve the traffic monitoring performance. Interestingly, with appropriate weights between the two objectives, monitoring performance and robotaxi average speed can be improved simultaneously. This suggests better network monitoring leads to more accurate traffic state prediction and improved mobility. This win-win situation could incentivize robotaxi operators to contribute their vehicles as drive-by sensors for traffic monitoring.

==> text/Case_Study.tex <==
\section{Case Study}

\subsection{Experimental Setting}
To evaluate the proposed routing for monitoring framework, a SUMO simulation model is developed in this study. A $5\times5$ grid network, consisting of $40$ bidirectional two-lane links and $25$ four-approach intersections is shown in Figure \ref{fig:grid_network}. The network is further expanded with 20 entry and exit links in SUMO for vehicle generation and departure, as shown in Figure ~\ref{fig:sumo_network}. The distance between intersections is set to $400$ meters. The entry and exit links are set to 240 meters. %Additionally, for simulation purposes, $20$ short links of $240$ meters are added at the network boundaries to facilitate vehicle loading and discharging as shown in Fig.~\ref{fig:sumo_network}. 
The corresponding CTM network is shown in Figure \ref{fig:ctm_network}. The cell length is set to 80 meters, calculated by the time resolution (i.e., 5s) and the free flow travel time in SUMO (i.e., 16 m/s). Each internal link contains 7 cells as shown in Figure \ref{fig:ctm_link} and each entry/exit link contains 3 cells, with a total number of 760 cells in the network.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/optim_network.png}
    \caption{A $5\times 5$ Grid Network}
    \label{fig:grid_network}
\end{figure}

Other settings in the SUMO simulation are listed below:
\begin{enumerate}
    \item \textbf{Traffic Demand Generation}: A total of $16$ origin–destination (OD) pairs are set in the grid network following a "diagonal pattern" that make vehicles travel from one side of the network to the opposite side. In SUMO simulation, vehicles are generated at the entry links and demand is set to a fixed flow rate of $350 \,\mathrm{veh/h}$ for each link. All OD pairs and their corresponding traffic demands are shown in Table \ref{Table:od-demand}. The same flow rate is applied to the CTM source cells. 
    \item \textbf{Simulation Setting}: The total simulation duration is set to  $5400\,\mathrm{s}$, with the first $1800\,\mathrm{s}$ used for warm up. The remaining one-hour simulation ($3600\,\mathrm{s}$) time is used for data collection and performance evaluation.
    \item \textbf{No Lane Changing Zone}: A no lane changing zone of 80 meters is set before the stop bar of each intersection. All CAVs are not allowed to change lanes within the last $80\,\mathrm{m}$ of the approaching links, which is the same length as the intersection cell in the CTM network.
    \item  \textbf{Traffic Signal Setting}: Fixed-time traffic signal is applied at all $25$ intersections in the network. A four-phase split signal timing plan is adopted because of the shared lanes at the intersection, as shown in Figure \ref{fig:phase_setting}. The cycle length is set to 100s and evenly distributed to the four phases.
    %same-approach phases with the same signal split($25\,\mathrm{s}$) are applied (Figure \ref{fig:phase_setting}), with a length of $100\,\mathrm{s}$ for one cycle. 
    % \item \textbf{Benchmark Routing Generation}: The dynamic user equilibrium (DUE) tool in SUMO \textcolor{red}{ref!!!!!!!!!!!!!!!!!!!!} is applied to generate benchmark routing strategies. This tools performs a DUE model to all the traffic (both background traffic and CAVs). The optimal routing planning generated from this model is recoded as the baseline. 
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figure/phase setting.png}
    \caption{Fixed-time signal timing plan for intersections}
    \label{fig:phase_setting}
\end{figure}


As indicated in Figure \ref{fig:main_workflow}, different components in the proposed framework run at different time resolutions.  The SUMO network runs at a time resolution of $0.1\,\mathrm{s}$. The CTM model updates the traffic state every $5\,\mathrm{s}$ in simulation time. Every $100\,\mathrm{s}$ (i.e., every 20 CTM steps), the dynamic routing model is triggered to update routes for all CAVs in the network. In time steps when routing is not triggered, CTM only predicts one step ahead to keep up with the simulation environment. In time steps when the dynamic routing model is executed, CTM calculates traffic states for the next 300 steps, which is equivalent to the planning horizon $T$, to provide time dependent travel time of each cell.

    % \item \textbf{Vehicle Travel Budget}: To provide flexibilities as well as avoid looping. A travel budget is given for CAVs during the simulation. For example, budget=2 means the vehicle is allowed to choose it feasible routes whose length is no more than 2 links plus the shortest path from its current location. Given the grid network is studied in this paper, it means the vehicle is able to \textit{deroute} one more node to cover more. Since CAVs under different O-D demand have different shortest path length and 


% might be too complicated.....
% \subsection{Feasible Routes Generation}
\subsection{CAV Travel Budget}
Although Equation \ref{eqa:single visit} prevents CAV subtour in the formulation, subtours may still be generated from later planning results because each route planning is executed independently and uses the CAVs current location as the origin. Especially when coverage weight $\alpha_2$ is set to a large value, the optimization model may encourage CAVs to de-route as much as possible and result in continuous subtours. To avoid this situation, "travel budget" of each CAV before each route planning is assigned considering three factors: \textbf{Single de-routing budget}, 
\textbf{Total de-routing budget} and \textbf{Maximum travel distance}. The single de-routing budget means the extra travel distance, in terms of number of links, that a CAV can choose compared to its distance shortest path in one route planning. For example, if the de-routing budget equals to 2, it means that the CAV is allowed to travel two more links from its shortest distance paths. Since the study area is a grid network, whenever a vehicle tries to de-route, the additional links must be even numbers. The total de-routing budget limits the total number of additional links that a CAV can de-route during the entire trip across multiple route planning horizons. If a CAV reaches the total de-routing budget, only shortest distance paths are available to make sure it can arrive its destination as soon as possible. The maximum travel distance limits the maximum number of links a CAV can travel during the entire trip. If the travel distance before the current planning horizon plus the remaining distance shortest path reach this threshold, de-route is forbidden for this CAV, even if single/maximum de-routing budget are not met. 

Given the O-D demand in Table \ref{Table:od-demand} and network typology, The travel budget parameters are set as below:

\begin{itemize}
    \item Single de-routing budget is set to $2$ when the number of links in the shortest distance path is smaller or equal to $6$, and $0$ otherwise.
    \item Total de-routing budget is set to $12$.
    \item The Maximum travel distance is set to $18$.
\end{itemize}


Before solving the dynamic routing problem every 100s, a set of feasible routes are generated for each CAV based on the above mentioned rules. 

\begin{table}[h]
\centering
\caption{Origin-destination (OD) Demand for Each Node in Grid Network}
\label{Table:od-demand}
\begin{tabular}{ccl @{\hspace{2cm}} ccl} 
\hline\hline
\textbf{Origin} & \textbf{Destination} & \textbf{Flow Rate} & \textbf{Origin} & \textbf{Destination} & \textbf{Flow Rate} \\
\hline
$A1$ & $E5$ & $700 \ \mathrm{veh/h}$ & $E3$ & $A3$ & $350 \ \mathrm{veh/h}$ \\
$A2$ & $E4$ & $350 \ \mathrm{veh/h}$ & $E2$ & $A4$ & $350 \ \mathrm{veh/h}$ \\
$A3$ & $E3$ & $350 \ \mathrm{veh/h}$ & $E1$ & $A5$ & $700 \ \mathrm{veh/h}$ \\
$A4$ & $E2$ & $350 \ \mathrm{veh/h}$ & $D1$ & $B5$ & $350 \ \mathrm{veh/h}$ \\
$A5$ & $E1$ & $700 \ \mathrm{veh/h}$ & $C1$ & $C5$ & $350 \ \mathrm{veh/h}$ \\
$B5$ & $D1$ & $350 \ \mathrm{veh/h}$ & $B1$ & $D5$ & $350 \ \mathrm{veh/h}$ \\
$C5$ & $C1$ & $350 \ \mathrm{veh/h}$ & $E4$ & $A2$ & $350 \ \mathrm{veh/h}$ \\
$D5$ & $B1$ & $350 \ \mathrm{veh/h}$ & $E5$ & $A1$ & $700 \ \mathrm{veh/h}$ \\
\hline\hline
\end{tabular}
\end{table}



%\subsection{Benchmark}

\begin{figure}[H]
    \centering
    \begin{subcaptionbox}{SUMO Network\label{fig:sumo_network}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/sumo_network.png}}
    \end{subcaptionbox}
    \begin{subcaptionbox}{CTM Network\label{fig:ctm_network}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_network.png}}
    \end{subcaptionbox}
    \hfill
    \caption{5 by 5 Urban Network for SUMO and CTM Representation}
    \label{fig:sumo_ctm_network}
\end{figure}

\subsection{Results and Analysis}

Experiments are conducted under three CAV penetration rates (2\%, 5\%, and 10\%) and four weight combinations of $\alpha_1$ and $\alpha_2$ ($(1:0)$, $(1:10^4)$, $(1:10^5)$ and $(1:10^6)$). The three penetration rates represent an early CAV deployment stage. The $(1:0)$ weight combination makes CAVs only aim to minimize travel time and the $(1:10^6)$ weight combination means that CAVs prioritize the network coverage objective. The other two weight combinations balance the two objectives. Two additional experiments are conducted with two weight combinations without any travel budget ("$(1:0)$ no budget" and "$(1:10^6)$ no budget"), in which CAVs can only choose shortest distance paths. Experiment results are reported in Table \ref{Table:350_result}.




%as shown in Equation~\ref{eqa:obj_function}, which represent the importance of travel time and average network convergence, respectively. Specifically, the tested parameter combinations include $\alpha_1:\alpha_2 = (1:0)$, $(1:10^4)$, $(1:10^5)$ and $(1:10^6)$. At each time step, the occupancy status of each cell is recorded as 1 if one or more CAVs are present; otherwise, it is recorded as 0. In summary, the evaluation metrics include the average travel time of both CAVs and background vehicle (BV), as well as the spatiotemporal coverage across the evaluation period. A total of three penetration levels are considered ($2\%$, $5\%$, and $10\%$) with a link demand of $350 \,\mathrm{veh/hour}$, with an additional group of testing in 10\% penetration rate when the travel budget is set to zero. The details are shown in Table \ref{Table:350_result}.


\begin{table}[h]
\caption{Experiment Results Under Different CAV Penetration Rates and Routing Strategies}
\label{Table:350_result}
\begin{center}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{lccccccc} 
\hline\hline
\textbf{Case($\alpha_1$:$\alpha_2$)} & 
\makecell{\textbf{Penetration} \\ \textbf{Rate}} & 
\makecell{\textbf{CAV Avg.} \\ \textbf{Travel Time}} & 
\makecell{\textbf{CAV Avg.} \\ \textbf{Travel Distance}} & 
\makecell{\textbf{CAV Avg.} \\ \textbf{Travel Speed}} &
\makecell{\textbf{BV Avg.} \\ \textbf{Travel Time}} & 
\makecell{\textbf{BV Avg.} \\ \textbf{Travel Distance}} & 
\textbf{Coverage} \\
\hline
% Benchmark & $2\%$ & 608.18 & 2976.2 & 613.83 & 2981.6 & 2.43\% \\
$1:0$  & $2\%$ & 640.69 & 3041.2 & 4.75& 635.87 & 3000.47 & 2.27\% \\
$1:10^{4}$ & $2\%$ & 625.99 & \textbf{3014.7} & 4.82 &631.50 & 3001.4 & 2.77\% \\ %2.768
$1:10^{5}$ & $2\%$ & \textbf{613.86} & 3028.7 & 4.93 &632.70 & 3002.0 & 2.77\% \\ %2.770
$1:10^{6}$ & $2\%$ & 814.02 & 4070.6 & 5.00 &636.08 & 3000.0 & \textbf{3.59\%} \\
\hline
% Benchmark & $5\%$ & 603.44 & 2941.4 & 604.22 & 2985.8 & 6.02\% \\
$1:0$  & $5\%$ & 626.80 & \textbf{3094.2} & 4.93 &611.07 & 2995.4 & 6.34\% \\
$1:10^{4}$ & $5\%$ & 628.31 & 3103.0 & 4.94 & 608.06 & 2995.7 & 6.53\% \\
$1:10^{5}$ & $5\%$ & \textbf{614.22} & 3109.3 & 5.06 & 606.37 & 2995.5 & 6.70\% \\
$1:10^{6}$ & $5\%$ & 757.84 & 3786.9 & 5.00 &616.49 & 2996.5 & \textbf{8.18\%} \\
% \textcolor{red}{$10^{-1}:10^{6}$ } & $5\%$ & \textcolor{red}{728.05} & \textcolor{red}{3637.4} & \textcolor{red}{609.45} & \textcolor{red}{2986.5} & \textbf{7.25\%} \\
\hline
% Benchmark & $10\%$ & 616.02 & 2971.9 & 623.66 & 2981.2 & 11.36\% \\
$1:0$ & $10\%$ & 680.86 & \textbf{3082.0} & 4.53 &652.78 & 2994.3 & 11.35\% \\
$1:10^{4}$  & $10\%$ & 668.76 & 3086.5 & 4.62 &645.80 & 2994.9 & 11.83\% \\
$1:10^{5}$  & $10\%$ & \textbf{646.03} & 3084.4 & 4.77 &640.91 & 2994.3 & 12.58\% \\
$1:10^{6}$ & $10\%$ & 710.87 & 3469.5 & 4.88 &644.20 & 2993.9 & \textbf{14.45\%} \\
\hline
$1:0\ \text{no budget}$ & $10\%$ & 659.01 & \textbf{2948.6} & 4.47 &647.42 & 2994.3 & 11.05\% \\
$1:10^6\ \text{no budget}$ & $10\%$ & \textbf{615.21} & 2986.4 & \textbf{4.85} &636.41 & 2993.8 & \textbf{12.95\%} \\
% $0.01:10^{6} \ \text{no budget}$ & $10\%$ & 614.46 & 2983.8 & 637.19 & 2996.3 & \textbf{12.92\%} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}


It is observed that under each CAV penetration rate, the background vehicle's travel time keeps relatively consistent regardless of the CAV routing strategies. This result further confirms that under low penetration rates, CAV routing does not impact the overall traffic. From the CAV's perspective, with the increase of coverage weight $\alpha_2$, the spatiotemporal network coverage also increases under all penetration rates. It can be seen that CAVs' average travel time decreases when the weight of $\alpha_2$ increases to $10^4$ and $10^5$. Meanwhile, the CAV average travel distances remain similar. This result indicates that CAVs are able to find better paths (in terms of travel time) without de-routing (i.e., increasing travel distance). It is possibly because increased coverage also improves the accuracy of the CTM-based traffic state estimation model, by replacing more cells with true CAV observations. A more accurate CTM leads to a more accurate time dependent travel time estimation and thus improves the route selection. This is an interesting finding that the aim of improving traffic monitoring performance can also benefit individual vehicles, which is a win-win situation. However, when the coverage weight keeps increasing to $10^6$, both the network coverage and the CAV average travel time and travel distance are significantly increased, indicating that more coverage is achieved by scarifying travel time. Figure \ref{fig:duration-route_his_budget} compares the average CAV travel distance distribution and travel time distribution under the two extreme weight combinations. The figure clearly shows that under the $1:10^6$ weight combination, CAVs choose longer routes with longer travel time.

%Testing results without travel budget also prove raising coverage weight will increase the converge rate. Based on the result, different strategies are applied to increase coverage rate compares with given travel budget and no travel budget. For cases when travel budget is provided, the maximized coverage rate is reached with the exchange of adding travel distance. On the other hand, when no budget is provided, the coverage rate is also increased by proper allocate the vehicle routes. This is also demonstrated in Figure~\ref{fig:duration-route_his_budget} and Figure~\ref{fig:duration-route_his_nobudget}. Both figures show the distributions of vehicle counts based on travel distance and travel time. The comparison is made under a $10\%$ penetration rate. Two weight parameter combinations are considered: $\alpha_1:\alpha_2=1:0$ and $\alpha_1:\alpha_2=1:10^6$. Blue bars correspond to the case with no coverage consideration ($\alpha_2 = 0$), while yellow bars correspond to the case with maximum coverage consideration ($\alpha_2=10^6$).

In the two experiments where no travel budget is allowed, all CAVs are expected to choose one of the shortest distance paths. Given the O-D demand in Table~\ref{Table:od-demand} and the network topology in Figure~\ref{fig:grid_network}, there are only three possible travel distances in this scenario ($3680 \mathrm{m}$, $2880 \mathrm{m}$, and $2080 \mathrm{m}$). As shown in Figure \ref{fig:routelth_his_10} and the last two rows in Table \ref{Table:350_result}, the CAV average travel distances are similar. However, both the average travel time and the network coverage are improved. Figure \ref{fig:duration_his_10} shows that that under the $(1:0)$ weight combination, the travel time distribution has a longer tail with more vehicles with higher travel times (>800s), compared with the $(1:10^6)$ scenario. Similar as in other experiments, increased network coverage may lead to better traffic state estimation model, which helps CAVs to choose better routes. Furthermore, the cell occupation distributions are compared under these two experiments, as shown in Figure \ref{fig:cell_occupation_his_5}. The horizontal axis is the number of time steps occupied by CAVs of a specific cell and the vertical axis is the frequency. It can be seen that the number of zero occupation cells is significantly reduced under the $(1:10^6)$ scenario, which implies more evenly distributed CAVs across the network over time, given the same travel distance budget.

%The routing algorithms can only extend some of the CAVs with shorter path to improve the coverage shown as Figure \ref{fig:routelth_his_10} However, if the travel budget is given, some of the CAVs will extend their total travel distance to reach higher coverage as shown in Figure \ref{fig:routelth_his_10b}. Nevertheless, the change of travel time distribution also shows the routing algorithm will balance the total travel time over coverage rate. Specifically, when there is no travel budget allowed, the travel time distribution is more clustered with fewer long trip. This proves the routing algorithm turns out to reach a system-optimal states to boost the coverage rather than simply re-routing a small portion of vehicle to reach the max coverage. 

%Additionally, result in Table \ref{Table:350_result} also shows the average travel time decreases with the increasing of spatiotemporal coverage. More clustering on travel time distribution in Figure \ref{fig:duration_his_10} shows the same pattern. It is possibly because the improvement of coverage improves the accuracy for traffic state estimation, which is used to predict the future travel time before each routing assignment. Thus there are fewer vehicles have the potential gap between its actual travel time and its planned time. So fewer \textit{extreme} long trips appear in that case, making the overall travel time distribution more cluster as a normal distribution. This implies the improvement of cell converge rate buffs the qualities on traffic state estimation result. 

% Figure~\ref{fig:routelth_his_10} demonstrates that the proposed routing algorithm selectively extends the route for CAVs with shorter paths in order to improve coverage, rather than uniformly extending all vehicle routes. Furthermore, Figure~\ref{fig:duration_his_10} confirms that no \textit{extreme} rerouting occurs, indicating that coverage improvements are achieved without excessive detours. \textcolor{red}{This also proves the algorithm follows the equality????????} 



\begin{figure}[h]
    \centering
     \begin{subcaptionbox}{Travel Distance Distribution\label{fig:routelth_his_10b}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_vis/routeleng_10b_his_0vs1e6.png}}
    \end{subcaptionbox}
    \begin{subcaptionbox}{Travel Time Distribution\label{fig:duration_his_10b}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_vis/duration_10b_his_0vs1e6.png}}
    \end{subcaptionbox} 
    \hfill
    \caption{CAV Travel Distance and Travel Time Distribution with Travel Budget  (Pr=10\%)}
    \label{fig:duration-route_his_budget}
\end{figure}


\begin{figure}[h]
    \centering
     \begin{subcaptionbox}{Travel Distance Distribution\label{fig:routelth_his_10}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_vis/routeleng_his_0vs1e6.png}}
    \end{subcaptionbox}
    \begin{subcaptionbox}{Travel Time Distribution\label{fig:duration_his_10}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_vis/duration_his_0vs1e6.png}}
    \end{subcaptionbox} 
    \hfill
    \caption{CAV Travel Distance and Travel Time Distribution without Travel Budget (Pr=10\%)}
    \label{fig:duration-route_his_nobudget}
\end{figure}



%Figure \ref{fig:cell_occupation_his_5} shows the histogram for cell occupation number across the network during the evaluation period ($720 \,\mathrm{steps}$) under weight parameter $\alpha_1:\alpha_2=1:0$ and $\alpha_1:\alpha_2=1:10^6$. The height of the bars indicates the frequency of the cells that being occupied by different time steps. It can be observed that the distributions turns out to be flattened with the increasing of coverage rate. 
 

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figure/ctm_vis/cell_occupation_his.png}
    \caption{Cell Occupation Distribution without Travel Budget (Pr=10\%)}
    \label{fig:cell_occupation_his_5}
\end{figure}

\subsection{Implications of Real-world Deployment}
Given the successful deployment of robotaxi services such as Waymo and Tesla in several US cities, CAV fleets operated by mobility companies represent ideal platforms for implementing the proposed routing for monitoring framework, due to their wide availability, extensive network access, and ability to choose dynamic routes while serving passengers. These robotaxis are highly automated vehicles and are equipped with perception sensors suitable for traffic monitoring. The embedded communication capabilities, typically via celluar networks, enable real-time transmission of detected surrounding traffic information to a central server. As our preliminary experiment results show that, in certain scenarios, improved collective traffic monitoring performance can also benefit individual vehicles by providing more accurate navigation information and reduce travel time. Even in other scenarios that longer routes may be required to optimize network coverage, incentive-based programs can be developed to encourage passengers to accept a long route for rewards (e.g., discounts, or gift cards). Importantly, it is likely that only a subset of vehicles would need to take longer routes to achieve sufficient monitoring improvements, while other vehicles could benefit from the enhanced situational awareness without deviating from their optimal paths. 





% From the testing results, we have observed the increasing the coverage weight leads to a higher coverage rate across all penetration levels by selectively extending a certain portion of vehicle trips to improve overall system performance. When a travel budget is applied, the system achieve more raise than no budget is applied, as the routing algorithm has more flexibility in selecting routes. However, the distributions of travel distance shown in Figure~\ref{fig:routelth_his_10} and Figure~\ref{fig:routelth_his_10b} indicate that the algorithm does not blindly maximize travel distance to achieve coverage. 

==> text/Conclusion.tex <==
\section{Conclusion and Future Work}
In this paper, we proposed a novel framework that integrated microscopic simulation, traffic state estimation, and dynamic vehicle routing to improve cooperative perception based traffic monitoring under low CAV penetration rates. A SUMO-based simulation environment was developed to provide the traffic environment including both background vehicles and CAVs. A cell-based network typology was applied to support both traffic state estimation and network coverage modeling. The Cell Transmission Model (CTM) wass employed to estimate and predict traffic states and generate time-dependent travel costs for routing optimization. A MILP formulation was then developed to optimize CAV routes under a rolling horizon scheme. The objective function considered both CAV total travel time and network coverage to represent traffic monitor performance. A case study was conducted in a $5 \times 5$ grid network with symmetric O-D demand and fixed-time traffic signals. Three CAV penetration rates were evaluated: $2\,\%$, $5\,\%$, and $10\,\%$, each tested with multiple weight parameter combinations. %Additionally, a conditional travel budget is introduced to prevent infinite routing loops while maintaining routing flexibility.
Results showed that increasing the weight of coverage in the objective function could effectively change the routing strategy so that CAVs would cover more unobserved cells. When proper weights are assigned between the two objectives or with limited routing budget, the average travel time of CAVs could also be reduced, possibly because increased network coverage could also improve the accuracy of the traffic state estimation and prediction model.

Future work includes 1) improving the accuracy of the traffic state estimation/prediction model; 2) designing more efficient solution algorithms for the dynamic vehicle routing model; and 3) incorporating realistic CAV perception systems by integrating the proposed framework with a high-fidelity simulator (e.g., CARLA).


%If travel budget is provide, the optimal routing algorithm turns to extending the travel distance. However, if the budget restrictions are applied, the optimal routing strategies can also improve the network coverage. Additionally, we also observed the increasing of coverage rate, with same penetration rate, could improve the CAV travel time. This is possibly because increasing coverage enhances traffic state estimation accuracy given more real-time information is provide. The future work includes more comprehensive testing on different demand flow rate, weight parameter combination and the prediction accuracy for CTM model.

==> text/Literature_Review.tex <==
\section{Literature Review}
\subsection{Traffic Monitoring}

% from different trajectory pattern. 
% 1. loop detector ( Yan zhao, PINN loop dector)
% 2. cv
% 3. cav cp

Traffic monitoring aims at estimating, predicting, or reconstructing spatiotemporal traffic states (e.g., flow, density, and speed) with single or multi-modal data sources. Serving as the input for traffic monitoring models, traffic data collection methods vary by sensor modality.

Loop detectors are the most widely deployed sensor type for traffic data collection and monitoring, which provide continuous temporal coverage at specific locations. Loop detector data contains occupancy and flow information, which can be used to further infer other traffic parameters such as travel time. \citet{dailey1993cross} proposed to use cross-correlation of flow counts between upstream and downstream loop detectors to estimate the average link travel time. The method adaptively selects lags and yields robust results under congested conditions. Later on, \citet{jin2006stochastic} introduced a probabilistic regression model considering the variability of travel time as random variables. Advanced methods such as machine learning models are developed to estimate traffic states based on loop detector data. For example, \citet{shi2021pidl} developed a physics-informed neural network (PINN) framework that integrates first and second order traffic flow models with a neural network. With data collected from loop detectors, the method is able to learn a function form of the fundamental diagram high estimation accuracy. 

Utilizing data from probe vehicles (i.e. CV, CAV) to estimated traffic states has been extensively studied in the past decades. Compared to loop detector data, trajectory data from probe vehicles provides spatially continuous observations of vehicle movements. Due to limited penetration rates of probe vehicles, different methods have been developed to estimate complete traffic states from partial observations \cite{Yuan2024GAI, han2021estimation}, or even reconstruct all vehicle trajectories \cite{sun2013vehicle, chen2022vehicle, zhang2025vehicle}. Specifically, Han and Ahn \cite{han2021estimation} developed both Bayesian inference and deep learning models to estimate traffic flow using CAV headway data. Their results show that the Bayesian approach performs reliably at low CAV penetration (as low as 10\%), while deep learning models achieve higher accuracy at moderate-to-high penetration levels. 

Under cooperative perception, CAVs share their detection results with each other or with the infrastructure, which greatly improve the traffic monitoring efficiency. A much lower CAV penetration rate is needed to collect equivalent data than those from probe vehicles \cite{Li_Han_Ma_2022, Xia_Meng_Han_Li_Tsukiji_Xu_Zheng_Ma_2023, Cai_Qu_Gao_Chen_2023}. For example, \cite{cao2022analytical} shows that less than 10\% of CAVs are able to observe more than 50\% of total vehicles on average. \citep{chen2022cooperative} also obtained similar results that 5\% of CAVs plus an infrastructure Lidar sensor could reach nearly 50\% of equivalent probe vehicle market penetration rate. The cooperative perception based data collection mechanism also brings two new challenges. First, the observed vehicles are clustered around the CAV rather than randomly distributed across the road segments as seen in data collected from the probe vehicles. Second, if CAVs are clustered together, a great portion of the collected data from each CAV is redundant. To improve traffic monitoring efficiency, CAVs need to be distributed sparsely within the network, each covering non overlapping spatial and temporal areas and intervals. In this study, we focus on addressing the second challenge with the proposed routing for monitoring framework.      

\subsection{Vehicle Routing Problem}
Vehicle Routing Problem (VRP) is a widely studied problem, which focuses on finding the minimum cost routes for a fleet of vehicles with certain constraints. In a mixed traffic condition with CAVs and human driven vehicles (HDVs), exist studies aim at optimize the routes of CAVs to improve the traffic network performance \cite{zhang2018mitigating, guo2021mixed}. For example, \citet{zhang2018mitigating} proposed a routing scheme to control a small portion of CAVs and bring the system close to system optimum. The work proposed in \cite{guo2021mixed} has a similar objective but further considers instantaneous dynamic user equilibrium (IDUE) for HDV and dynamic system optimal (DSO) for CAVs. This work, along with others such as ~\cite{psaraftis1995dynamic, ouertani2023dynamic}, incorporate time-dependent link travel times into the routing framework, which can be considered as a Dynamic Vehicle Routing Problem (DVRP). Similarly, in \cite{Li_Mirchandani_Zhou_2015}, the time dependent travel time is represented by a space-phase-time (SPT) hypernetwork. Notable, this studies not only optimizes routes for vehicles, but jointly optimizes traffic signals. More work about time-dependent vehicle routing problems can be found in \cite{gendreau2015time}. From the methodology perspective, \citet{munari2016generalized} reviewed two major forms of vehicle routing problem formulation, link-based and path-based. The link-based formulation considers link travel time and use decision variables (i.e., whether to traverse a specific link) to associate links in a network graph \cite{Li_Mirchandani_Zhou_2015}, while the path-based formulation defines decision variable based on the paths and optimizes routes from a feasible path set. %\citet{bezzi2023route} applies a route-based formulation solving electric vehicle routing problem with mixed-integer linear programming. 


%Other than this, with the nature that traffic state information is updated to the decision maker concurrently with the determination of the routes ~\cite{psaraftis1995dynamic}, dynamic vehicle routing problem has long being studies for years with different solving method ~\cite{ouertani2023dynamic}. In the real world, information is often affected by uncertainty and may be only partially observed. For the Vehicle Routing Problem (VRP), two critical dimensions contribute to this dynamic nature: information quality and information evolution~\cite{Abbatecola_Fanti_Ukovich_2016}. Our study addresses this gap by expanding the spatiotemporal coverage of CAVs, which increases real-time observations across the traffic network. In addition, a structured traffic state estimation model, such as the Cell Transmission Model (CTM), helps ensure the accuracy of future prediction results.


%Existing Studies on certain vehicle routing problems does not specifically designed for traffic monitoring senarios, Yet it still offers insights on this study. On one hand, several studies in transportation areas model the routing for CAV with a Dynamic Vehicle Routing Problem \cite{zhang2018mitigating, Guo_Ban_Aziz_2021}. Further more, some other researches about vehicle routing with multi-objective formulation such as traffic signal optimization \cite{Smith_2015, de2020multi}. The study \cite{Smith_2015} proposes a novel dynamic model that jointly integrates traffic signal control (TSC) and route choice within a unified optimization framework. It models the routing choice in path-based flows coupled with signal timing as a dynamic system, where route choice evolves through a restricted proportional adjustment process. With a theoretical guarantees, under mild conditions, the joint dynamics converge to a Wardrop equilibrium. \citep{Li_Mirchandani_Zhou_2015} propose a unified framework for simultaneous route guidance and traffic signal optimization using a space–phase–time hypernetwork. Their model captures the spatiotemporal interaction between routing and signal control within a single network representation. By applying Lagrangian relaxation, the problem is decomposed into tractable subproblems, enabling scalable optimization and near-optimal system performance in real-time applications. This study provides a good template to formulate the dynamic vehicle routing with time-depend link travel time. But the lack of modeling on traffic monitoring from the coverage perspective is still required to to solved.

In terms of the objective of the vehicle routing problem, most studies focus on reducing total travel cost (e.g., distance, travel time \cite{zhang2018mitigating, guo2021mixed, Li_Mirchandani_Zhou_2015}) or network congestion level (e.g., total queue length \cite{de2020multi}). Recent works start to include other objectives such as sustainability (e.g., energy consumption) and fairness (equity). For instance, in the context of electric vehicles, \citep{Cai2023Energy} introduced a multi-objective VRP variant addressing energy consumption under traffic congestion, time windows, and simultaneous pickup-and-delivery settings. This model jointly minimizes total cost and maximizes customer satisfaction, while incorporating a dynamic energy consumption model considering vehicle speed and load. As for equity, fairness has been included in DVRP. \citep{Kang2024Fairness} proposed a two-sided fairness framework for DVRP, introducing a fairness-aware genetic algorithm (2FairGA) that balances utilities between both service providers and customers. Additionally, workload equity (i.e., equally distribution of workload among all vehicles) in VRP has been studied. \citep{Matl2016Survey} analyzed various equity functions for balanced route workloads, highlighting how non-monotonic measures can produce inconsistent outcomes, while \citep{Nekooghadirli2022Multiperiod} showed that multi-period workload equity can coexist with near-optimal routing costs over longer planning horizons.

In summary, existing studies have explored modeling DVRPs with various objectives.
%, which are partially aligned with the goals of our research. For instance, the dynamic routing studies provide modeling approaches that adapt network typology and spatiotemporal traveling, while multi-objective formulations offer valuable insights into balancing different objective components within a single function. 
However, to the best of our knowledge, there are very few studies that consider traffic monitoring in the dynamic vehicle routing framework, especially under the CAV cooperative perception setting. This study tries to fill this research gap.




% On the other hand, studies from the related field also provide insights to model the vehicle routing dynamically. For example, OP and Travel Salesman Problem are two similar terms. Specifically, Orienteering Problem (OP) represents the routing problem in which the goal is to determine a subset of nodes to visit, and in which order, so that the total collected score is maximized and a given time budget is not exceeded \citep{gunawan2016orienteering}. This is similar to the traffic monitoring objective since we also want the moving vehicle to visit different places as much as possible with given budget. Travel Salesman Problem (TSP) shares the same insights with the traffic monitoring perspective as well since each moving CAV can be seen as a "salesman" who is willing to visit a sequential set of links. \cite{diaby2006traveling, Schneider_2002}


% \textcolor{red}{add routing + energy/equity, }
% \subsection{Sensor Placement Problem}

==> text/Methodology.tex <==
\section{Methodology}
\subsection{Framework Overview}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figure/Figure 2_updated.png}
    \caption{Overview of the routing for traffic monitoring framework}
    \label{fig:main_workflow}
\end{figure}


An overview of the proposed routing for monitoring framework is illustrated in Figure ~\ref{fig:main_workflow}. We use SUMO as the microscopic simulation platform in this study. Two types of vehicles are generated in SUMO, background vehicles (BV) and CAVs. BVs serve as background traffic while CAVs are able to perform traffic monitoring tasks by observing surrounding vehicles within a predefined detection range. A cell-based network typology is designed and each link is divided into seven cells as shown in Figure~\ref{fig:ctm_link}. This cell-based network typology is combined with the CAV's location in SUMO to determine whether a cell is occupied by the CAV. If a cell is occupied by one or more CAVs, it is considered being observed. An observed cell provides complete traffic data (e.g., average speed, and density/number of vehicles). The same cell-based network typology is also applied to construct the CTM for traffic state estimation. The cell length is set to be the same as the typical detection range of the CAV (e.g., 80 meters). The CTM runs in parallel with the SUMO simulation and estimate/deduce current traffic states based on historical traffic data (e.g., turning ratio at the intersection cells, and average traffic demand at source cells) and CAV observations. In addition, the CTM is also responsible for predicting future traffic states. It runs beyond the current time to generate cell-based traffic states for $T$ more time steps, where $T$ is the planning horizon in the Dynamic Vehicle Routing model. The predicted traffic states (i.e., density of each cell at each time step) are stored in a spatiotemporal matrix by cell and time indexes, from which the time-dependent travel time can be derived. Finally, when the Dynamic Vehicle Routing model is activated, it requires inputs including the network typology, current CAV locations and O-D information, time dependent cell travel time, and predetermined optimization hyper-parameters. The Dynamic Vehicle Routing model is formulated as a mixed-integer linear programming (MILP) model to find optimal routes for all CAVs in the network. The objective function aims to minimize total CAV travel time while maximizing network coverage or equivalently maximizing the total number of observed cells during the planning horizon. A rolling horizon scheme is employed to solve the MILP iteratively, allowing the model to accommodate changing traffic conditions and update monitoring results. The optimized CAV routing decisions are then applied to the SUMO simulation after each planning horizon for execution.

Note that the SUMO simulation, the CTM and the routing algorithm are executed at different resolutions. In our setting, SUMO is executed every 0.1s, which is a typical time step for microscopic simulation. The CTM is executed every 5s, which is calculated based on the desgined cell length and the free flow speed in the network. Finally, the dynamic routing algorithm is executed every 100s to balance the computational complexity and the solution quality.

Major assumptions of this study are listed below.

\begin{enumerate}
    \item It is assumed that CAVs' routing decisions do not affect the background traffic's routing decisions and corresponding time dependent travel time, under very low penetration rates (e.g., less than $10\%$).
    \item The travel time within the intersection area is ignored when calculating the total travel time of a specific route, but the delay caused by the traffic signals are considered. %For both CAVs and background traffic, there are no transition time between cells. That is to say in CTM network, the geometry of intersection will be ignored.
    \item A central controller has access to all CAVs' real-time information (i.e., location at each time step) and is responsible for assigning the routes to the CAVs. All CAVs follow the exact routes assigned by the central controller. %shared information about the entire network prior to routing. At the beginning of each planning horizon, CAVs are assumed to start from the beginning of their respective cells, based on their current positions in the network.
 
\end{enumerate}



\subsection{Cell Transmission Model for Network Traffic}

The CTM is a first order discrete approximation of the LWR model \cite{lighthill1955kinematic, richards1956shock}, proposed by Daganzo in 1994 ~\cite{daganzo1994ctm1}. The model assumes a triangular fundamental diagram and represents a road segment with consecutive homogeneous sections. The cell length $l$ is calculated as $l=v_{f}\cdot\Delta t$, in which $v_f$ refers to the free flow speed and $\Delta t$ is the time step. Later, Daganzo extended the model to represent network traffic, which allows it to model urban networks with signalized intersections \cite{daganzo1995ctm2}. 

\begin{figure}[H]
    \centering
    \begin{subcaptionbox}{Link-level cell typology\label{fig:ctm_link}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_link_combined.png}}
    \end{subcaptionbox}
    \hfill
    \begin{subcaptionbox}{Intersection-level cell typology\label{fig:ctm_inter}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/ctm_inter_source.png}}
    \end{subcaptionbox}
    \caption{Network CTM Representation}
    \label{fig:ctm_typology}
\end{figure}




% \begin{figure}[h]
%     \centering
%     \begin{subcaptionbox}{Ordinary cell\label{fig:ctm_str_nm}}[0.48\linewidth]
%         {\includegraphics[width=\linewidth]{figure/ctm_structure_st.png}}
%     \end{subcaptionbox}
%     \hfill
%     \begin{subcaptionbox}{Merging cell\label{fig:ctm_str_mg}}[0.23\linewidth]
%         {\includegraphics[width=\linewidth]{figure/ctm_structure_mg.png}}
%     \end{subcaptionbox}
%     \hfill
%     \begin{subcaptionbox}{Diverging cell\label{fig:ctm_str_div}}[0.23\linewidth]
%         {\includegraphics[width=\linewidth]{figure/ctm_structure_div.png}}
%     \end{subcaptionbox}
%     \caption{Cell Transmission Model for Network Traffic}
%     \label{fig:ctm_structure}
% \end{figure}

% For ordinary cell that have one upstream and one downstream cells, as shown in Figure \ref{fig:ctm_str_nm}, the change of vehicle number for given cell $i$ between step $t$ and $t+1$ comply with \ref{eqa:ctm_flow_nm}, \textcolor{green}{in which $n_i(t)$ represents the number of vehicles present in cell $i$ at time step $t$; and $y_{i-1, i}(t)$ represents the vehicle flow form cell $i-1$ to $i$ at time step $t$, For $i \in Z^{+}, t \in Z^{+}$:}

% \begin{equation}
%     n_i(t+1) = n_i(t) + y_{i-1, i}(t)-y_{i, i+1}(t)
%     \label{eqa:ctm_flow_nm}
% \end{equation}

% As for cell $i$ refers to the source and sink cells at the entry and exit of the network. The change of vehicle number patter comply with \ref{eqa:ctm_flow_source} and \ref{eqa:ctm_flow_sink} respectively. Noted that $d_i$ refers to the demand for cell $i$ at time $t$.

% \begin{equation}
%     n_i(t+1) = n_i(t) + d_i(t)-y_{i, i+1}(t)
%     \label{eqa:ctm_flow_source}
% \end{equation}

% \begin{equation}
%     n_i(t+1) = n_i(t) + y_{i-1, i}(t)
%     \label{eqa:ctm_flow_sink}
% \end{equation}

% Figure \ref{fig:ctm_str_mg} and \ref{fig:ctm_str_div} illustrate the merging and diverging system for CTM network ~\cite{daganzo1995cell}. Noted that Bk and Ek are denoted as the first two cells and Ck is denoted as the \textit{other} cells (i.e the third cell). In a merging system, Ck denotes the second upstream merging cell; whereas in a diverging system, Ck refers to the second downstream diverging cell. The sending and receiving function for each cells are denoted as $S_{Bk}$ and $R_{Bk}$ taking cell Bk as an example; and the actual number of vehicle transmitted through the cell bound are denoted as $y$ respectively. 

% The merging maneuver may have two conditions determined by whether the downstream cell EK  is able to take it upstream flow. For the cases that downstream cell Ek is not over saturated, saying if $R_{Ek} \geq S_{Bk}+S_{Ck}$, it complies to \ref{eqa:ctm_merge_nocongest}. 

% \begin{equation}
%     \begin{cases}
%         y_bk=S_{Bk} \\
%         y_ck=S_{Ck}
%     \end{cases}
%     \label{eqa:ctm_merge_nocongest}
% \end{equation}

% For the cases that cell Ek is over saturated when $R_{Ek} < S_{Bk}+S_{Ck}$, it complies to \ref{eqa:ctm_merge_congest}. Assuming that a fraction $p_{bk}$ of the vehicles comes from Bk and the remainder ($p_{ck}$) from Ck, where $p_{bk}+p_{ck}=1$.   

% \begin{equation}
%     \begin{cases}
%         y_{bk}=\texttt{mid}\{S_{Bk}, R_{Ek}-S_{Ck}, p_{bk}\cdot R_{Ek}\} \\
%         y_{ck}=\texttt{mid}\{S_{Ck}, R_{Ek}-S_{Bk}, p_{bk}\cdot R_{Ek}\} \\
%     \end{cases}
%     \label{eqa:ctm_merge_congest}
% \end{equation}

% For diverging maneuver, cell Bk is the only upstream cell that transmits vehicle to cell Ck and Ek. The outbound vehicle number of cell Bk is denoted as $y_{bk}$, which is bound by \ref{eqa:ctm_dive_1}. The fraction $p_{ck}$$p_{ek}$ indicate the divergent proportion from Bk and $p_{ck}+p_{ek}=1$

% \begin{equation}
%     y_{bk} = \texttt{min}\{S_{Bk}, \frac{R_{Ck}}{p_{ck}}, \frac{R_{Ek}}{p_{ek}}\}
%     \label{eqa:ctm_dive_1}
% \end{equation}

% Then the downstream flow can be divided by the divergent proportion by \ref{eqa:ctm_div_2}

% \begin{equation}
% \begin{cases}
%     y_{ck}=p_{ck}\cdot y_{bk} \\
%     y_{ek}=p_{ek}\cdot y_{bk}
% \end{cases}
% \label{eqa:ctm_div_2}
% \end{equation}

Six different types of cells are defined to represent a signalized urban network: ordinary cell, merging cell, diverging cell, source cell, sink cell and intersection cell. The flow dynamics between cells all follow the definitions in \cite{daganzo1994ctm1, daganzo1995ctm2}. Then the urban network is decomposed into a cell-level representation. Figure \ref{fig:ctm_typology} illustrates the design of cells for links and intersections. We consider a typical grid network with equal link length so that the cell configuration in each link is the same. For example, in Figure \ref{fig:ctm_link}, for a two-lane link, we use two separate cells at the entrance (C1 and C2) to receive the arriving flow from the upstream links.  The flow merges in the middle of the link (C3, C4, and C5). Then, C5 diverges to C6 and C7, mimicking the channelization at the intersection. Note that the capacity of C3, C4 and, C5 is twice as of other cells. 
%Thus cell $1$, $2$, and $3$ will be set as merging cells at cell level. Symmetrically, the last two segments in the link, cell $5$, $6$, and$7$ are set as diverge cells. 
At the intersection, it is assumed that the left lane is a shared lane for left turning and through traffic while the right lane is also a shared lane for right turning and through traffic, as illustrated in Figure \ref{fig:ctm_inter}. The diverging ratios for cells $5$, $6$, and $7$ can be estimated based on historical flow data (i.e., turning ratio) of the corresponding link, assuming that through traffic is evenly distributed in the left and right lanes. %For instance, let $a_l$, $a_t$, and $a_r$ denote the historical flow rates for left-turn, through, and right-turn movements, respectively. Then, based on the lane-movement allocation shown in Figure \ref{fig:ctm_link}, the left lane is able to turn left and through while the right lane is set to turn right and through. The diverging ratio for cell $6$ is calculated by the proportion of $a_l$ and $0.5\cdot a_{t}$ to the downstream cells, which are index as cell $1$ for the other links (Figure \ref{fig:ctm_inter}). cell $7$ hold the same diverging ratio based on $a_r$ and $0.5\cdot a_{t}$. This is based on the assumptions that the through movement will equally separated to two lanes near stop line. Similarly, the diverging ratio for cell $5$ is calculated as $p_{56} = \frac{a_l + 0.5 \cdot a_t}{a_l + a_t + a_r}$, and for cell $7$ as $p_{57} = \frac{a_r + 0.5 \cdot a_t}{a_l + a_t + a_r}$. In this way, the merging proportion of cell $3$ can be determined by the cells from upstream links based on the connection typologies shown in Figure \ref{fig:ctm_inter}.
A four-phase fixed-time signal plan is applied at each intersection with a split phasing  (i.e., traffic signals at each approach take turns to be green). 
%The split phasing is adopted because shared lanes usually require split phasing so that vehicles traveling to different directions do not block each other.
Finally, cells 6 and 7 are considered as intersection cells, whose outflows are controlled by signal status.

%. 2) It also prevents the \textcolor{red}{cascading effect} for Cells near the intersection. According to the cell connections in Figure \ref{fig:ctm_inter}, for example, starting for southbound diverging cell $7$, the out flow will be one of the merging flow for cell $2$ on west and south links. And it has the possibilities to influence another merging flow for these two cells according to \ref{eqa:ctm_merge_congest}. In this way, it leads to a cascading consequences on the diverging flow for eastbound cell $7$ an westbound cell $7$ according to \ref{eqa:ctm_dive_1}. And this effect will further expand to four approaches in this intersection. However, if the traffic signal is set to the same approaches simultaneously, cell $1$ and $2$ in four approaches will become \textit{ordinary cell} given the other connection is disabled by traffic signals. Thus, in terms of integrating traffic signals into the intersection, it is only required to multiple a binary signal flag $\theta_{i}(t) =1$ to the outflows for cell $6$ and $7$. The signal flag complies to \ref{eqa:signal_flag}.

% \begin{equation}
%     \theta_{i}(t)=
%     \begin{cases}
%         1 \quad if \ signal \ is\ green \\
%         0 \quad if \ signal \ is\ red \\
%     \end{cases}
%     \label{eqa:signal_flag}
% \end{equation}

% Additional assumptions regarding CTM and vehicle routing modeling are listed below:

% \begin{enumerate}
%     \item The cell length are designed to be $80m$. It will be denoted as fully observed on traffic state whenever there is one or more CAVs in the cell. 
%     \item The route choices of CAVs will not affect the background vehicle condition given the low penetration rate. 
%     \item All CAVs are able to access the shared information for entire network before routing.
% \end{enumerate}





\subsection{Dynamic Vehicle Routing Model Formulation}
The objective of the dynamic vehicle routing model aims to generate optimal routes for all CAVs in the network considering the maximization of spatiotemporal network coverage and minimization of total CAV travel time. Main notations used in the formulation are shown in Table \ref{Table:notations}.

\begin{table}[h]
\begin{flushleft}
\caption{Variables and Notations}
\label{Table:notations}
\begin{tabular}{lp{14cm}}
\hline\hline
\textbf{Notation} & \textbf{Meaning} \\
\hline
% variables
$A$ & Set of CAVs\\
$I$ & Set of cells in the network\\
$E$ & Set of edges in the network \\
$T$ & Planning horizon \\
$x_{i, t}^{a}$               & Binary variable, equals to 1 if vehicle $a$ enters cell $i$ at time $t$, and 0 otherwise\\
$z_{i, j, t, s}^{a}$            & Binary variable, equals to 1 if vehicle $a$ enters cell $i$ at time $t$ and leaves cell $i$ at time $s$, heading to cell $j$, and 0 otherwise\\
$y_{i}^{t}$ & Binary variable, equals to 1 if cell $i$ is occupied by any CAV(s) at time $t$, and 0 otherwise\\
$\omega_{i, t}^{a}$ & Binary variable, equals to 1 if vehicle $a$ occupies cell $i$ at time $t$, and 0 otherwise\\

$c_{i}^{t}$ & Parameter, time dependent travel time of cell $i$ for vehicles entering at time $t$ \\ 
$\Pi_{i, j}$ & Binary parameter for network typology, equals to 1 when cell $i$ is connected to cell $j$, and 0 otherwise, $(i, j) \in E$ \\

$o(a)$ & Origin cell or the starting cell at the beginning of planning horizon of vehicle $a$ \\
$d(a)$ & Destination cell of vehicle $a$ \\
$M$ & A sufficiently big number \\
\hline\hline
\end{tabular}
\end{flushleft}
\end{table}

We model the urban traffic network as a directed graph $G(I, E)$. Each cell in the CTM representation $i\in I$ is considered as a node and the connection between cells $i$ and $j$, $(i,j) \in E$ is considered as a directed edge. Time is discretized into steps, and the planning horizon $T$ represents the total number of time steps. The time resolution in the dynamic routing model is set to be the same as in the CTM and the planning horizon is predefined and should be long enough for all CAVs in the network to reach their destinations.
%Three dimensions: number of vehicle, number of nodes, and planning horizon, denoted as $A$, $I$, $T$ are considered in the formulaiton. The formulation is modeled by cell-based network so each cell will be denoted as a node during the modeling, while the time step shares the same length with CTM modeling. 
Four primary variables are designed to formulate the problem. $x_{i,t}^{a}$ is used to represent selected cells in a CAV route and the entry time $t$ is used to find the corresponding time dependent travel time $c_i^t$. 
%route selection and entry time of each so the value equals to 1 whenever vehicle $a$ choose to enter cell $i$ starting from time $t$. 
Variable $z_{i,j,t,s}^{a}$ further expands the dimension of $x_{i,t}^{a}$ to include the connecting cell(s) $j$ and the departure time $s$, which is mainly used to formulate the flow conservation, ensuring the selected cells consist of a feasible path.
Variable $\omega_{i, t}^{a}$ is designed for vehicle-level cell occupation and $y_{i}^{t}$ indicates the cell-level spatiotemporal occupation, which is used to calculate the coverage term in the objective function.
%and the value equals to $1$ when there are one or more vehicles in cell $i$ at time $t$. 
%Furthermore, in order to track the vehicle route selection and vehicle-specific coverage on cells, $z$ and $\omega$ are designed. $z_{i,j,t,s}^{a}$ expand its index to a travel spatiotemporal index $\{i,j,t,s\}$. $z_{i,j,t,s}^{a}=1$ when vehicle $a$ arrives at node $i$ at time $t$ and depart at time $s$ heading to node $j$, otherwise $z_{i,j,t,s}^{a}=1$. Given there are not transition time between nodes, time $s$ is also the arriving time for node $j$. This allows the decision variable to track the route in time-space network. Variable $\omega_{i, t}^{a}$ is designed to represent the occupation for vehicle $a$ given time $t$ at cell $i$. $\omega=1$ whenever vehicle $a$ is traveling in cell $i$ at time $t$, otherwise $\omega=0$.





%by the density matrix from CTM prediction (denoted as $k_{i}^{t}$). With the parameters on fundamental diagram, a cell-level spatiotemporal speed matrix is calculated (denoted as $v_{i}^{t}$). Then for each cell $i$ at time $t$, starting from step $t$, the remaining distance will be continuously reduced by $v_{i}^{t} \cdot \Delta t$ from cell length $FD.length$ until it is less or equal to $0$. The total steps will be the travel cost $c_{i}^{t}$ for cell $i$ at time $t$. Details are shown in \ref{alg:get_cost_ctm}.  
%$\Pi_{i, j}=1$ whenever cell $i$ has a feasible connection to cell $j$, otherwise $\Pi_{i, j}=0$, and it is based on the typology for the cell-based network. 





% \begin{algorithm}[H]
% \caption{Time-dependent Travel Time Calculation}
% \label{alg:get_cost_ctm}
% \KwIn{Vehicle count matrix $\mathbf{N}$, fundamental diagram parameters $\text{FD}$}
% \KwOut{time cost matrix $\mathbf{C}$}

% \For{each cell $i$}{
%     \For{each time step $j$}{
%         \eIf{$K_{i,j} \leq \frac{\text{FD}.q_{\max}}{\text{FD}.v_f}$}{
%             $Q_{i,j} \leftarrow \text{FD}.v_f \cdot K_{i,j}$\;
%         }{
%             $Q_{i,j} \leftarrow -\text{FD}.w \cdot (K_{i,j} - \text{FD}.k_{\text{jam}})$\;
%         }
%     }
% }

% Initialize time cost matrix: $\mathbf{C} \leftarrow \mathbf{1}$\;

% \For{each cell $i$}{
%     \For{each time step $t$}{
%         \If{$K_{i,t} \neq 0$}{
%             $V_{i,t} \leftarrow Q_{i,t} / K_{i,t}$\;
%         }
%         Initialize: $\text{step} \leftarrow 0$, $\text{dist} \leftarrow \text{FD}.\text{length}$\;
%         \For{future time steps $t' = t, \dots, T$}{
%             $\text{dist} \leftarrow \text{dist} - V_{i,t'} \cdot \text{FD}.\delta_t$\;
%             $\text{step} \leftarrow \text{step} + 1$\;
%             \If{$\text{dist} \leq 0$}{
%                 $C_{i,t} \leftarrow \text{step}$\;
%                 \textbf{break}\;
%             }
%         }
%     }
% }

% \Return $\mathbf{C}$\;

% \end{algorithm}


% For the objective function, total travel time for all CAVs are considered as the first components while the spatiotemporal network coverage is considered as the second term. The objective for this MILP formulation is to minimize the total travel time for all CAVs and maximized the spatiotemporal coverage at the same time. So the second term is used to measure the total coverage of the CAVs in next $T$ steps. Noted that $T$ stands for the total time steps planned in this optimization formulation, thus in practice, the value of $T$ should be bigger than the longest possible travel time. Notations are shown in Table \ref{Table:notations}. 
% \subsubsection{Parameter calculation}

% The MILP formulation requies some optimization parameters from CTM component. 
% \textcolor{red}{add calculation logic for $c_{i}^{t}$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Objective function}
The objective function contains two terms which represent total CAV travel time and spatiotemporal network coverage, with corresponding weights $\alpha_{1}$ and $\alpha_{2}$. The total CAV travel time is calculated as the summation of all cell traverse time of all CAVs in the network. The network coverage is calculated by the summation of cell occupation $y_i^{t}$ over time, and normalized by total time steps and total number of cells. Note that since both $T$ and $I$ are constants, the normalization will not impact the solution. Since the overarching goal is to maximize network coverage and minimizing total travel time at the same time, the values of $\alpha_{1}$ and $\alpha_{2}$ should be properly selected to keep a balance between the two objectives. The objective function is shown in Equation~\ref{eqa:obj_function}.

\begin{linenomath}
    \begin{equation}
        \text{min} \ \  \alpha_{1}\sum_{a\in A}\sum_{i\in I, t\in T}{c^{t}_{i} \times x_{i, t}^{a}} - \alpha_{2}\frac{\sum_{i \in I, t \in T}{y_{i}^{t}}}{I \times T}
        \label{eqa:obj_function}
    \end{equation}
\end{linenomath}

\subsubsection{Connection between \texorpdfstring{$x$}{x} and \texorpdfstring{$z$}{z}}
As variable  $x_{i,t}^{a}$ only determines the entry time of cell $i$ while $z_{i, j, t, s}^{a}$ also determines the departure time $s$ and the downstream cell $j$ of the same cell. Equation \ref{eqa:x-z condition} depicts that when a vehicle enters cell $i$, it can only have one combination of departure time and downstream cell. Equation \ref{eqa:cell connection} considers the network typology $\Pi_{i, j}$. Only a connected downstream cell of cell $i$ can be chosen. 
%$z$ indicates the arrival on cell $i$ at time $t$ and leave at time $s$ but $x$ only indicates the arrival on cell $i$ at time $t$, $x_{i,t}^{a}$ should be equal to the summation of $z_{i, j, t, s}^{a}$ for all $j$ and $s$ shown in Equation \ref{eqa:x-z condition}
 % x-z condition
\begin{equation}
    x_{i, t}^{a} = \sum_{j}\sum_{s}{z_{i, j, t, s}^{a}} \quad \forall a \in A\quad i\in I \quad t\in T
\label{eqa:x-z condition}
\end{equation}

%Given $z_{i, j, t, s}^{a}$ contains the heading cell index compared with $x_{i,t}^{a}$, network typology are also considered shown as \ref{eqa:cell connection}. If $\Pi_{i,j}=0$, which means there are no feasible connections between cell $i$ and cell $j$, $z_{i, j, t, s}^{a}$ is forced to be 0 given its nature of binary integers. Additionally, since signal information has been considered in CTM and reflect to the time-dependent cost $c_{i}^{t}$ with big number. this constraint only considers the connections from network typology. 

%Net typology 
\begin{equation}
    z_{i,j,t,s}^{a} \leq \Pi_{i, j} * x_{i,t}^{a} \quad \forall a \in A \quad i \in I \quad t \in T \\
\label{eqa:cell connection}
\end{equation}



\subsubsection{Network flow constraints}

The flow conservation constraint in Equation \ref{eqa:flow_conservation2} guarantees that selected cells with associated entry and departure times consist of a time-continuous feasible path. 
% More specifically, if vehicle $a$ enters cell $i$ at time $t$ and leaves at time $s$ towards cell $j$, then this constraint assigns $z_{j, k, s, r}^a$ equals to 1. 
Note that this constraint also applies to intersection cells because the travel time within the intersection is not considered, and waiting time at traffic signals is included in the cell travel time $c_i^t$. Equations \ref{eqa:flow_conservation1} and \ref{eqa:flow_conservation3} ensure the vehicle starts at the origin cell and reaches the destination cell.
Furthermore, Equation \ref{eqa:temporal uniqueness} constraints that one vehicle cannot enter multiple cells at the same time and Equation \ref{eqa:single visit} limits each cell can be visited by each vehicle only one time (subtour elimination). 

%Noted that vehicles will use the sink cells as their destination cell when generating $d(a)$ from SUMO. That means if $i=d(a)$, $j$ does not exist at all. So the flow conservation will not necessarily to be hold. 


\begin{equation}
    \sum_{j\in I,\ s\in T}z_{i, j, t, s}^{a} = 1  \quad \quad \text{if} \ i=o(a) \ \& \ t=0 \quad \quad \quad \quad \forall a\in A \quad t,s\in T
    \label{eqa:flow_conservation1}
\end{equation}

\begin{equation}
    \sum_{i\in I, \ t \in T}z_{i, j, t, s}^{a} - \sum_{k \in I,\ r \in T}z_{j, k, s, r}^{a} =  0  \quad \quad \text{if} \ j \neq o(a) \ \& \ j \neq d(a)  \quad \quad \quad \quad \forall a\in A \quad t,s,r\in T
    \label{eqa:flow_conservation2}
\end{equation}

\begin{equation}
    \sum_{i\in I,\ t,s \in T}z_{i, j, t, s}^{a} =1 \quad \quad \text{if} \ j = d(a)  \quad \quad \quad \quad \forall a\in A \quad t,s\in T
    \label{eqa:flow_conservation3}
\end{equation}


% \begin{align}
%     \begin{cases}
%     \sum_{j\in I,\ s\in T}z_{i, j, t, s}^{a} = 1  \quad \quad \text{if} \ i=o(a) \ \& \ t=0 \\
%     \sum_{i\in I, \ t \in T}z_{i, j, t, s}^{a} - \sum_{k \in I,\ r \in T}z_{j, k, s, r}^{a} =  0  \quad \quad \text{if} \ j \neq o(a) \ \& \ j \neq d(a)\\
%     \sum_{i\in I,\ t,s \in T}z_{i, j, t, s}^{a} =1 \quad \quad \text{if} \ j = d(a)
%     \end{cases}
%     \quad \quad \forall a\in A \quad t,s,r\in T
%     \label{eqa:flow_conservation}
% \end{align}


% \begin{align}
%     x^{a}_{i,t} = 1 \quad \forall  i=o(a)
%     \label{eqa:flow_conservation_2}
% \end{align}



%\subsubsection{Vehicle spatiotemporal constraints}
%Temporal uniqueness constraint \ref{eqa:temporal uniqueness} is set to avoid duplicated appearance for one vehicle on different cells at the same time. Aiming at reduce the search complexity for the model and avoid looping, \ref{eqa:single visit} forces vehicles only visit each cell once during its whole trip. 

% temproal uniquness
\begin{equation}
    \sum_{i \in I}{x_{i, t}^{a}} \leq 1 \quad \forall a \in A, \ t \in T
\label{eqa:temporal uniqueness}
\end{equation}

%one visit bound
\begin{equation}
    \sum_{t \in T}x_{i, t}^{a} \leq 1 \quad \forall a \in A, \ i \in I
\label{eqa:single visit}
\end{equation}

\subsubsection{Vehicle-level network occupation constraints}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figure/omg-x.png}
    \caption{Relationship between $\omega$ and $x$}
    \label{fig:omg-x relation}
\end{figure}


We use variable $\omega$ to model the vehicle-level occupation of cells. The value of $\omega_{i,t}^{a}$ is determined by both $x_{i, t}^{a}$ and time dependent travel time $c_{i}^{t}$. The relation between $\omega$ and $x$ is shown in Figure \ref{fig:omg-x relation}. Equation \ref{eqa:omg-x cond0} illustrates if vehicle $a$ never visits cell $i$, then the occupation should be set to 0. If vehicle $a$ visits cell $i$ at certain time point $t$ (i.e., $x_{i, t}^{a}=1$), then this constraints is released and Equations \ref{eqa:omg-x cond1} to \ref{eqa:omg-x cond3} become effective. These three constraints collectively regulate the values of $\omega$ should be one from time $t$ to time $t+c_i^t-1$, and zero otherwise. 
%Determined by $x$, $\forall a, i, t$, if $x_{i, t}^{a}=0$, $\omega_{i, t}^{a} =0$. This means vehicle $a$ has never visited cell $i$ along time. \ref{eqa:omg-x cond0} bounded this condition. On the other hand, if $\exists a, i, t, \ x_{i,t}^{a}=1$, the mapping between $x$ and $\omega$ would become complicated. Figure \ref{fig:omg-x relation} shows the case when vehicle $a$ arrives in cell $i$ at time $k$, along with the time dimension, only $x_{i, k}^{a}=1$. However, as of $\omega$, the value should be equal to $1$ when $t\in [k,\  k+c_{i}^{k}-1]$. Additionally, $\omega$ should be equal $0$ when $t\in [0,\  k-1]$ and $t\in [k+c_{i}^{k}, T]$ assuming  $T$ is the max value of time step. \ref{eqa:omg-x cond1} to \ref{eqa:omg-x cond3} bounded this logic with given $\omega$ is a binary integer. 
These constraints are further linearized using the big-M method as shown in Equations \ref{eqa:omg-x-1:linear1} to \ref{eqa:omg-x-3:linear2}.


\begin{equation}
    \omega_{i, t}^{a} \leq \sum_{t \in T}{x_{i, t}^{a}} \quad \forall a \in A, i \in I, t \in T
    \label{eqa:omg-x cond0}
\end{equation}

 %   if $x_{i, t}^{a}=1$: 

\begin{equation}
    \sum_{0\leq k \leq t-1}{\omega_{i, k}^{a}}=0 \quad \forall i \in I, a \in A, t \in T
\label{eqa:omg-x cond1}
\end{equation}

\begin{equation}
    \sum_{t\leq k \leq t+c_{i}^{t}}{\omega_{i, k}^{a}}=c_{i}^{t} \quad \forall i \in I, a \in A, t \in T
\label{eqa:omg-x cond2}
\end{equation}

\begin{equation}
    \sum_{t+c_{i}^{t}+1\leq k < T}{\omega_{i, k}^{a}}=0 \quad \forall i \in I, a \in A, t \in T
\label{eqa:omg-x cond3}
\end{equation}


%The linearization of \ref{eqa:omg-x cond1} to \ref{eqa:omg-y cond} by Big M method is shown as below:
 
%Linearized form for \ref{eqa:omg-x cond1} is listed below:

\begin{equation}
    \sum_{0\leq k \leq t-1}{\omega_{i, t}^{a}} \geq 0 
    \label{eqa:omg-x-1:linear1}
\end{equation}

\begin{equation}
    \sum_{0\leq k \leq t-1}{\omega_{i, t}^{a}} \leq  M\times (1-x_{i, t}^{a})
    \label{eqa:omg-x-1:linear2}
\end{equation}

%Linearized form for \ref{eqa:omg-x cond2} is listed below:

\begin{equation}
    \sum_{t\leq k \leq t+c_{i}^{t}}{\omega_{i, t}^{a}} \geq x_{i,t}^{a}\times c_{i, t} 
    \label{eqa:omg-x-2:linear1}
\end{equation}

\begin{equation}
    \sum_{t\leq k \leq t+c_{i}^{t}}{\omega_{i, t}^{a}} \leq x_{i,t}^{a}\times c_{i, t} + M\times (1-x_{i, t}^{a})
    \label{eqa:omg-x-2:linear2}
\end{equation}

%Linearized form for \ref{eqa:omg-x cond3} is listed below:

\begin{equation}
    \sum_{t+c_{i}^{t}+1\leq k < T}{\omega_{i, t}^{a}} \geq 0 
    \label{eqa:omg-x-3:linear1}
\end{equation}

\begin{equation}
    \sum_{t+c_{i}^{t}+1\leq k < T}{\omega_{i, t}^{a}} \leq  M\times (1-x_{i, t}^{a})
    \label{eqa:omg-x-3:linear2}
\end{equation}
        



\subsubsection{Cell-Level network occupation constraints (\texorpdfstring{$\omega$}{\omega} - \texorpdfstring{$y$}{y} relation)}

Converting vehicle-level occupation to cell-level occupation is necessary to handle the situation that multiple CAVs occupy a cell at the same time. We use variable $y_{i}^{t}$ indicates the occupation of cell $i$ at time $t$. Equation \ref{eqa:omg-y cond} states the relation and can be linearized to Equations \ref{eqa:omg-y:linear1} and \ref{eqa:omg-y:linear2} by the big-M method.
%Given $\omega_{i,t}^{a}$ is the vehicle specific occupation on cell $i$ at time $t$, \ref{eqa:omg-y cond} lets $y_{i}^{t}=1$ if there are more than one vehicles in cell $i$ at time $t$. Otherwise $y_{i}^{t}=0$. 
Note that in this study, we assume a perfect detection model so that all vehicles in the cell, if occupied by CAVs, can be observed. This can be further extended to more complicated and accurate detection models that consider detection accuracy and uncertainty. 

    \begin{align}
        y_{i}^{t} = 
        \begin{cases}
            1 \quad \text{if} \ \sum_{a}{\omega_{i, t}^{a}}  \geq 1 \\
            0 \quad \text{if} \ \sum_{a}{\omega_{i, t}^{a}} =0
        \end{cases}
    \label{eqa:omg-y cond}
\end{align}


%Linearized form for Equation \ref{eqa:omg-y cond} with Big M method is:
    \begin{equation}
        y_{i}^{t} \leq \sum_{a}{w_{i, t}^{a}}
        \label{eqa:omg-y:linear1}
    \end{equation}
        
    \begin{equation}
        M \times y_{i}^{t} \geq \sum_{a}{w_{i, t}^{a}}
        \label{eqa:omg-y:linear2}
    \end{equation}


In summary, the CAV dynamic routing model is formulated as a MILP problem (\textbf{P1}) as below:
%\begin{itemize}

    \textbf{Objective Function}: Equation \ref{eqa:obj_function}
    
    \textbf{Subjected to}: Equations \ref{eqa:x-z condition} - \ref{eqa:single visit}, \ref{eqa:omg-x-1:linear1} - \ref{eqa:omg-x-3:linear2}, and \ref{eqa:omg-y:linear1}-\ref{eqa:omg-y:linear2}
%\end{itemize}

One critical parameter that serves as the input to the model is the time dependent travel time $c_{i}^{t}$, which indicates the total time to traverse cell $i$ if a CAV enters the cell at time $t$. It is calculated based on the predicted traffic states from the CTM. Assume $k_{i}^{t}$ denotes the predicted density of cell $i$ at time $t$. The speed of the cell $v_{i}^{t}$ can be calculated using the triangle fundamental diagram. 

\begin{align}
    v_{i}^{t}=  
    \begin{cases}
        v_f \quad \text{if} \ 0 \leq k_{i}^{t} \leq k_c  \\
        w(k_j/k_{i}^{t}-1) \quad \text{if} \ k_c < k_{i}^{t} \leq k_j
    \end{cases}
    \label{eqa: cell_speed}
\end{align}

Then the travel distance $d_{i}^{t}$ at time $t$ can be calculated as

\begin{equation}
    d_{i}^{t}= v_{i}^{t} \times \Delta{t}
\label{eqa:dis}
\end{equation}

Where $w$ is the wave speed; $v_f$ is the free flow speed; $k_c$ is the critical density; and $k_j$ is the jam density. Finally, the time dependent travel time (or cell traverse time) $c_{i}^{t}$ can be calculated as the total time steps elapsed when the summation of $d_{i}^{t}$ from $t$ is greater than or equal to the cell length $l$.


%Not for the TRB version, but for the journal version, analyze the model complexity here. Then next talk about how to reduce that by fixing variable of z.



The complexity of the model comes mainly from $z_{i, j, t, s}^{a}$, which is a high-dimensional and very sparse matrix. 
%\subsubsection{Preset conditions for \texorpdfstring{$z$}{z} }
%For variable $z_{i, j, t, s}^{a}$, the subscript ${i,j,t,s}$ represents a time-space index from cell $i$ to cell $j$, starting at time $t$ and ending at time $s$. 
Considering time-dependent travel time $c_{i}^{t}$ and network typology, the value of $z$ can be one, only if conditions $s = t + c_{i}^{t}$ and $\Pi_{i,j}=1$ are satisfied. To reduce model complexity and improving solving efficiency, a subset of $z$ is set to zero as shown in Equation~\ref{eqa: z-preset}, which eliminates infeasible time-dependent arcs in advance.

\begin{align}
    z_{i,j,t,s}^{a} 
    \begin{cases}
        \leq 1 \quad \text{if} \ s=t+c_{i}^{t} \quad \& \quad \Pi_{i,j}=1\\
        =0 \quad \text{otherwise}
    \end{cases}
    \label{eqa: z-preset}
\end{align}

==> text/introduction.tex <==
\section{Introduction}

Urban traffic monitoring is essential for many transportation applications such as safety analysis \cite{yuan2018real}, congestion management \cite{liu2024traffic}, and incident response \cite{butilua2022urban}. Efficient monitoring also supports the deployment of advanced technologies such as ride hailing/sharing and autonomous driving, which rely on accurate traffic information to optimize routing and perform coordination. 
%Identifying traffic state has long been a critical task in the realm of intelligent transportation system (ITS) operations. It involves leveraging various types of sensors deployed throughout urban networks to collect data that reflect vehicle trajectories \cite{wang2024traffic, ref1a}, detect and monitor traffic congestion\cite{ref2a, ref2b, ref2c}, and provide real-time traffic information\textcolor{red}{ref3}. These insights can be further utilized to enhance roadway safety, improve traffic mobility, and increase overall travel efficiency.

Traditionally, infrastructure-based sensors such as inductive loop detectors embedded in pavement and roadside surveillance cameras have been widely deployed to collect traffic data, such as vehicle counts, average speeds, and average travel time. Yet the fixed locations of the sensors do not provide spatially continuous data. In recent years, the increasing deployment of Connected and Automated Vehicles (CAVs) have significantly changed the paradigm of traffic data collection. These vehicles, equipped with onboard sensors such as LiDAR, radar, and cameras, are capable of perceiving surrounding traffic with a high precision. With the support of Vehicle-to-Everything (V2X) communication technology, CAVs can share their perception data in real time and create a cooperative perception environment \cite{xiang2024v2x, chen2024cooperative}. Compared with probe vehicles which only report their own status, cooperative perception based traffic monitoring requires much lower market penetration rates and has great potential to be implemented at the early CAV deployment stage.  

Although cooperative perception based traffic monitoring offers high flexibility and scalability, the monitoring performance highly depends on the spatial-temporal distribution of the CAVs in the network. An illustrative example is provided in Figure \ref{fig:route_pattern}. Assuming three CAVs enter and leave the network at the same time, Figure \ref{fig:route_pattern1} shows when the three vehicles all choose their shortest path in terms of travel time or distance. During a certain time period, the green CAV and the blue CAV travel on the same link at the same time, generating redundant traffic data, and leaving the lower part of the network unobserved. However, if the blue vehicle chooses a longer route by turning right at the beginning as shown in Figure \ref{fig:route_pattern2}, the lower corridor can also be observed within certain time period, which improves the traffic monitoring performance by increased spatiotemporal sensor coverage. 

\begin{figure}[h]
    \centering
    \begin{subcaptionbox}{CAV routing solely based on travel time\label{fig:route_pattern1}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/cav_route_1.png}}
    \end{subcaptionbox}
    \hfill
    \begin{subcaptionbox}{CAV routing considering traffic monitoring\label{fig:route_pattern2}}[0.45\linewidth]
        {\includegraphics[width=\linewidth]{figure/cav_route_2.png}}
    \end{subcaptionbox}
    \caption{An Illustrative Example on CAV Routing Selection Considering Traffic Monitoring}
    \label{fig:route_pattern}
\end{figure}


This illustrative example demonstrates the relation (possibly the trade-off) between typical vehicle routing objectives (e.g., distance, travel time) and network traffic monitoring requirement, which motivates this study. While there exists rich literature in CAV based routing strategies, incorporating the traffic monitoring purpose into the routing framework, especially under the CAV cooperative perception environment, is still limited. 

Incorporating traffic monitoring poses new challenges to the vehicle routing problem, as listed below. 
\begin{itemize}
\item \textbf{Network Representation:} Most of existing vehicle routing methods are either path based \cite{bezzi2023route} or link based \cite{ran1996link, grosso2018mathematical}. \citet{munari2016generalized} gives a comprehensive review on both methods. However, due to the nature of the CAV-based monitoring, either path-based or link-based network representation is not sufficient. According to \cite{Arnold2019_3ddetection,xu2023v2v4real}, typical sensor detection ranges of a CAV are between $60 \,\mathrm{m}$ to $120\,\mathrm{m}$, which are significantly shorter than a typical link length in most road networks. As a result, when a CAV is traveling on a link, only a part of the link is observed. A higher granularity of road network representation is needed to realistically reflect the portion of network that are observed by CAVs.

\item \textbf{Performance Metric for Monitoring:} While minimizing travel time and/or travel distance are the most popular objectives for vehicle routing, it requires a new performance metric to indicate the efficiency of traffic monitoring. This metric should 1) directly reflect the quality of traffic monitoring; 2) be feasible to be computed from individual CAVs; and 3) collectively reflect the network wide performance.

\item \textbf{Time-dependent Dynamic Decision Making:} It is apparent that this CAV routing for monitoring framework should be dynamic. In contrast to static routing, routing decisions must be made frequently to adapt to evolving traffic conditions (e.g., time-dependent travel time) and monitoring results, leading to a high-dimensional decision space across time, vehicles, and network states. When combined with multiple objectives of travel efficiency and monitoring performance, the complexity of the problem increases significantly, requiring scalable and tractable solutions.

\end{itemize}


%Regarding the total travel time, the longer route may not result in higher travel time for two reasons: 1) the vehicle could arrive at the coordinated phase of the lower corridor due to traveling an extra link; and 2) with real-time detections provided by the CAV, the intersections along the corridor can provide better signal timing (e.g., adaptive signal control) to reduce delay. . With the dynamic nature of traffic conditions, floating vehicle-based monitoring brings greater flexibility, responsiveness, and more accurate real-time information for traffic management. These timely updates can be further utilized to enhance mobility and inform traffic control decisions.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figure/routing_covernot.png}
%     \caption{An Illustrative Example : Left: CAV routing solely based on travel time; Right: CAV routing considering traffic monitoring. }
%     \label{fig:route_pattern}
% \end{figure}




% In the foreseeable future, advanced vehicle platforms such as robot-taxi, ride-hailing services, and connected public buses are expected to be early adopters of routing-based traffic monitoring. Their widespread availability, extensive network access, and ability to dynamically route while picking up and dropping off passengers — coupled with modern communication technologies — make them ideal for this task. In this paper, we propose a novel routing-monitoring framework that leverages Dynamic Vehicle Routing Problem (DVRP) formulations integrated with the Cell Transmission Model (CTM) for real-time traffic state estimation. The objective of this study is to improve the spatiotemporal coverage of traffic monitoring across urban networks by utilizing mobile agents with optimized routing strategies. To achieve this goal, the main challenges are summarized as follows:

% \begin{itemize}
%     \item \textbf{Large-scale traffic state estimation}: The nature of Large-scale traffic state estimation requires significant computational and data acquisition to reconstruct the overall scope of the urban network. To get more accurate real-time estimation at large scale, the framework must efficiently integrate sparse and heterogeneous data while maintaining computational tractability. Balancing estimation accuracy, coverage, and real-time performance is therefore a core difficulty in large-scale deployments.
    
%     \item \textbf{The coupled conflicting objective between routing and monitoring}: The objectives of routing and monitoring are inherently coupled yet conflicting. On one hand, monitoring results directly determine the quality of traffic state information, which serves as input to the routing task. On the other hand, the routing decisions affect the monitoring outcome, as the positions of moving vehicles define where and when observations are made. However, while routing aims to minimize travel time, monitoring seeks to maximize spatiotemporal coverage of the network, often requiring vehicles to detour from the shortest path. This creates a fundamental trade-off between efficiency and information gain. How to model and balance these two interdependent yet conflicting objectives is a key challenge addressed in this study.

%     \item \textbf{The large scale of dynamic vehicle routing}: In contrast to static routing, dynamic policies must continuously adapt to evolving traffic conditions, leading to a high-dimensional decision space across time, vehicles, and network states. When combined with dual objectives of efficiency and monitoring, the complexity grows significantly, requiring scalable and tractable optimization methods to ensure real-time applicability.

% \end{itemize}




In this paper, we propose a novel dynamic CAV routing for monitoring framework to address all the aforementioned challenges. The proposed framework consists of three main components: \textit{Microscopic Simulation}, \textit{Traffic State Estimation} and \textit{Dynamic Vehicle Routing}. The microscopic simulation (i.e., SUMO) provides the traffic environment including both background vehicles and CAVs. For traffic state estimation, the Cell Transmission Model (CTM) is employed to predict future traffic states and calculate time dependent travel time for CAV routing decisions. Based on each CAV's location in the SUMO network, the portion of observable network (i.e., covered by the CAV's sensor range) can be obtained in terms of occupied cells over total cell number. Meanwhile, the observations from the CAVs are utilized to update the cell status in the CTM to improve its accuracy. The dynamic vehicle routing algorithm assigns optimal routes to all CAVs in the network that minimizes total travel times and maximizes spatiotemporal network coverage. Finally, the optimized CAV routes are given back to the microscopic simulation for execution during the next planning horizon. 
%The cell status for each planning interval will be defined as a spatiotemporal coverage matrix as the input for the dynamic routing problem. Utilizing the spatiotemporal coverage and the time-dependent travel time as two primary objectives, a mixed-integer linear programming (MILP) problem is formulated to solve the dynamic vehicle routing problem for all CAVs in the network simultaneously. 
% \textcolor{red}{maybe don't have to include the below words}\textcolor{red}{These components described above operate on different planning intervals. For example, as shown in Fig.~\ref{fig:main_workflow}, the SUMO network runs with a simulation step of $0.1\,\mathrm{s}$, while the CTM updates traffic state information every $5\,\mathrm{s}$ based on its time interval. For the Dynamic Vehicle Routing component, optimization is executed every $100\,\mathrm{s}$ to reflect broader planning horizons.}
Experiments from a 5 by 5 urban network under different CAV penetration rates show that considering the network monitoring purpose could effectively increase the spatiotemporal network coverage of CAVs when determining routes. Interestingly, with a properly selected weight ratio between two objectives or with travel budget restrictions, the optimal routing strategies can improve the network coverage and reduce CAV travel time simultaneously.   

% \sout{The cell length and time resolution of the CTM are designed based on the CAV detection range (e.g., 80 meters). As a result, the network typology is represented in cells and it is assumed that one cell is observed at time $t$ if there are one or more CAVs in the cell. This is achieved by tracking each CAV's location at each time step.  Finally, the performance metric of traffic monitoring is defined as the spatiotemporal coverage of the network by CAVs in each cell. Utilizing the spatiotemporal coverage and the time-dependent travel time as two primary objectives, a mixed-integer linear programming (MILP) problem is formulated to solve the dynamic vehicle routing problem for all CAVs in the network simultaneously. A rolling horizon scheme is applied to solve the MILP problem iteratively to incorporate changing traffic conditions and new monitoring results. An 5 by 5 grid network is built in SUMO to evaluate the proposed routing for monitoring framework} Results show....... 



To the best of our knowledge, this is one of the earliest works that integrates CAV based cooperative traffic monitoring with dynamic vehicle routing problem. The main contributions include:

\begin{enumerate}
    \item We propose a new CAV routing framework considering traffic monitoring performance in one explicit formulation.

    \item We apply CTM for traffic state prediction and road network representation and define traffic monitoring performance metric based on cell occupancy over time. 

    \item We integrate the proposed routing framework with microscopic simulation and evaluate its performance under various scenarios, demonstrating the applicability of our approach in future real-world implementation.
\end{enumerate}

The rest of the paper is organized as follows. Section 2 provides a brief literature review on related studies regarding traffic monitoring and vehicle routing. Section 3 introduces the methodologies including framework overview, CTM based traffic state estimation/prediction, and detailed formulations of the dynamic routing model. Section 4 presents a case study using a grid urban network, which evaluates the proposed framework under different CAV penetration rates and weight combinations. In addition, the implications of real-world implementation are discussed. Finally, Section 6 concludes the paper and lays out further research directions.


==> text_partB/notes.tex <==
% \begin{color}{green}
% \textbf{TRB Review Comments}
% However, there is a substantial gap in the explanation of the traffic state estimation. The authors clearly explained that when a CAV is present in a cell then the state is known, but do not explain how CTM proceeds when information is incomplete. This gap in explanation affect the validity of the main claim that coverage can improve CTM accuracy, sometimes leading to improved routing decisions. This is of critical importance and must be better explained in the future.

% I also have a few minor comments:
% \begin{enumerate}
%     \item The case study was very basic, and it would be helpful to see results on a larger and more realistic network to see whether these results extend to much more complicated traffic routing scenarios.
%     \item Assumption 1 seems very strong. Even with a small fleet size, routing decisions of CAVs could have a major impact on background traffic. Why not use something like citations \cite{zhang2018mitigating} and \cite{guo2021mixed}
%     \item Some coverage might matter more than others (the state of cells on opposite sides of the network could provide more information than neighboring cells), how could this be introduced into the objective?
%     \item Finally, can you explain more how the CAV travel budget might work when the network is not a grid and people generally care more about extra travel time than extra distance?
% \end{enumerate}

% \end{color}

% \begin{color}{blue}
% \textbf{Notes}
% \begin{enumerate}
%     \item We found CTM is hard to evaluate the dynamics for the network especially for the turning ratio in intersections. A possible todo is to change the diverge logic by breaking out the FIFO logic to verify this. 
%     % \item For CTM parameter calibration, we need to use entry link for calibration. 
%     \item We need to confirm the pattern of result still exists with new FD
%     \textcolor{red}{\item But it is still hard to argue that improving CTM by CAV observations will benefit the CAV Routing choice}
%     \item We need to prove the sensoring power distribution with our routing is greater than the benchmark case (using PNAS model in benchmark case). How to calculate the sensoring power? 
% \end{enumerate}
% \end{color}


% \begin{color}{purple}
% \textbf{TODO}
% \begin{enumerate}
%     % \item \sout{CTM logic need to complete, before that, we need to test the logics for diverging rules (when one of the downstream cells are full, fill the other one.)}
%     % \item \sout{Complexicity analysis}
%     % \item \sout{Toy network analysis}
%     % \item \sout{CTM evaluation results} 
%     % \item rerun experiment, update new values
%     % \item visulization: route heatmap, cell choice. 
%     % \item sensoring power calculation
%     \item \sout{Rewrite Introduction, include new story on robot taxi} 
%     \item \sout{update literature review first two parts} (when you update the literature review, focus on papers published in the past three years)
%     \item \sout{Add mobile sensor placement LR}
%     \item conclusion and final round review
% \end{enumerate}
% \end{color}
